Development of a front end ASIC for Dark Matter directional detection with MIMAC

A front end ASIC (BiCMOS-SiGe 0.35 \mum) has been developed within the framework of the MIMAC detector project, which aims at directional detection of non-baryonic Dark Matter. This search strategy requires 3D reconstruction of low energy (a few keV) tracks with a gaseous \muTPC. The development of this front end ASIC is a key point of the project, allowing the 3D track reconstruction. Each ASIC monitors 16 strips of pixels with charge preamplifiers and their time over threshold is provided in real time by current discriminators via two serializing LVDS links working at 320 MHz. The charge is summed over the 16 strips and provided via a shaper. These specifications have been chosen in order to build an auto triggered electronics. An acquisition board and the related software were developed in order to validate this methodology on a prototype chamber. The prototype detector presents an anode where 2 x 96 strips of pixels are monitored.

==> section3.tex <==
\section{toto}

